Optimal Online Discrepancy Minimization

We prove that there exists an online algorithm that for any sequence of vectors $v_1,\ldots,v_T \in \mathbb{R}^n$ with $\|v_i\|_2 \leq 1$, arriving one at a time, decides random signs $x_1,\ldots,x_T \in \{ -1,1\}$ so that for every $t \le T$, the prefix sum $\sum_{i=1}^t x_iv_i$ is $10$-subgaussian. This improves over the work of Alweiss, Liu and Sawhney who kept prefix sums $O(\sqrt{\log (nT)})$-subgaussian, and gives a $O(\sqrt{\log T})$ bound on the discrepancy $\max_{t \in T} \|\sum_{i=1}^t x_i v_i\|_\infty$. Our proof combines a generalization of Banaszczyk's prefix balancing result to trees with a cloning argument to find distributions rather than single colorings. We also show a matching $\Omega(\sqrt{\log T})$ strategy for an oblivious adversary.

==> Makefile <==
MAIN = onlineVectorBalancing
SOURCES = 

PAPER = letter

LATEX = latex
#BIBTEX = bibtex8 -W
BIBTEX = bibtex
DVIPS = dvips -f -Pcmz -G0 -t$(PAPER)
PSTOPDF = ps2pdf -dPDFsettings=/prepress -dAutoFilterColorImages=false \
  -dColorImageFilter=/FlateEncode
THUMBPDF = thumbpdf

ps: $(MAIN).ps

pdf: $(MAIN).pdf

$(MAIN).ps: $(MAIN).tex $(SOURCES)
#	$(LATEX) $(MAIN).tex
#	$(BIBTEX) $(MAIN)
	$(LATEX) $(MAIN).tex
	$(LATEX) $(MAIN).tex
	$(DVIPS) -o $(MAIN).ps $(MAIN).dvi

$(MAIN).pdf: $(MAIN).tex $(SOURCES)
	make ps
	$(PSTOPDF) $(MAIN).ps
	$(THUMBPDF) $(MAIN).pdf
	make ps
	$(PSTOPDF) $(MAIN).ps

clean:
	rm -rf $(MAIN).aux $(MAIN).dvi $(MAIN).log $(MAIN).blg $(MAIN).out *~

cleanall: clean
	rm -rf $(MAIN).bbl $(MAIN).ps $(MAIN).pdf

latexmk:
	latexmk -f -pdfps $(MAIN).tex
#	cp $(MAIN).pdf ~/Dropbox/CompiledPDFs/$(MAIN).pdf
#	cp $(MAIN).tex ~/Dropbox/Backup/TexFiles/$(MAIN).tex
#	/Applications/Adobe\ Reader.app/Contents/MacOS/AdobeReader $(MAIN).pdf &
#	/Applications/Adobe\ Acrobat\ Reader\ DC.app/Contents/MacOS/AdobeReader $(MAIN).pdf &
#	/Applications/Adobe\ Acrobat\ Reader.app/Contents/MacOS/AdobeReader $(MAIN).pdf &

thomas:
	latexmk -f -pdfps $(MAIN).tex
	cp $(MAIN).pdf ~/Dropbox/CompiledPDFs/$(MAIN).pdf
	cp $(MAIN).tex ~/Dropbox/Backup/TexFiles/$(MAIN).tex
#	/Applications/Adobe\ Reader.app/Contents/MacOS/AdobeReader $(MAIN).pdf &
#	/Applications/Adobe\ Acrobat\ Reader\ DC.app/Contents/MacOS/AdobeReader $(MAIN).pdf &
	/Applications/Adobe\ Acrobat\ Reader.app/Contents/MacOS/AdobeReader $(MAIN).pdf &

latexmk-do-not-open:
	latexmk -f -pdfps $(MAIN).tex
	cp $(MAIN).pdf ~/Dropbox/CompiledPDFs/$(MAIN).pdf
	cp $(MAIN).pdf ~/Dropbox/Backup/PDFs/$(MAIN)_`date +"%Y_%m_%d_TIME%H_%M"`.pdf
	cp $(MAIN).tex ~/Dropbox/Backup/TexFiles/$(MAIN).tex
	cp $(MAIN).tex ~/Dropbox/Backup/TexFiles/$(MAIN)_`date +"%Y_%m_%d_TIME%H_%M"`.tex

all:
	make cleanall
	make pdf
#	/Applications/Adobe\ Acrobat\ 9\ Pro/Adobe\ Acrobat\ Pro.app/Contents/MacOS/AdobeAcrobat $(MAIN).pdf &
	/Applications/Adobe\ Reader.app/Contents/MacOS/AdobeReader $(MAIN).pdf &

